Predicting the orientation of adsorbed proteins steered with electric fields using a simple electrostatic model

Under the most common experimental conditions, the adsorption of proteins to solid surfaces is an spontaneous process that leads to a rather compact layer of randomly oriented molecules. Due to the importance of this process for the development of catalytic surfaces, a number of existing computational and experimental approaches try to predict and control the orientation of such molecules. However, and despite their own advantages, these tend to be either too expensive computationally, or oversimplified, undermining their ability to predict the most appropriate experimental conditions to maximize the catalytic activity of adsorbed proteins. To address this current need, we present an efficient computational approach to model the behavior of proteins near surfaces in the presence of an external electric field, based on continuum electrostatics. Our model can not only estimate the overall affinity of the protein with the surface, but also their most likely orientation as a function of the potential applied. In this way, a rational selection of the potential can be performed to maximize the accessibility of the protein's active site to the solvent. The model relies on the Poisson-Boltzmann equation and was implemented in an extension of the code PyGBe that includes an external electric field, and renders the electrostatic component of the solvation free energy. To demonstrate the feasibility of this technique, we investigate the adsorption of trypsin onto a carbon electrode under potentiostatic conditions both numerically and experimentally. We found that even though the adsorption process is largely dominated by hydrophobic effects, the orientation of trypsin can be controlled through an external potential, influencing the position of the active sites, and resulting in an important change in the catalytic activity of the surface.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
